Deep Learning Quantification of Bainite Fractions from Optical Micrographs of Bearing Steel

Quantifying the bainite fraction in mixed bainite-martensite microstructures in bearing steels is important for process and quality control in bearing manufacture. In such steels, bainite and martensite exhibit strongly overlapping features in light-optical micrographs, often precluding reliable manual assessment. We present a deep learning regression method that predicts a dilatometry-derived reference bainite fraction directly from unsegmented optical images. Reference bainite fractions spanning the transformation range were generated by interrupting the bainitic transformation at points identified from the dilatometer length-change response. A deep neural network was trained using the captured optical micrographs and corresponding dilatometry-derived bainite fractions. The validation of the trained network covered held-out specimens within the same microscope domain, repeated metallographic preparation, and images from two additional microscopes. The lowest prediction errors were obtained within the original microscope domain while maintaining strong agreement after repeated metallographic preparation. Larger errors were observed for images acquired with the additional microscopes. The iterated mean filter reduced prediction errors for the two additional imaging workflows. These results demonstrate the feasibility of predicting reference bainite fractions directly from unsegmented optical images of high-carbon bearing steel. The approach requires neither image segmentation nor manual phase annotation.

==> Figures/Figure1_martensitic_expansion/heat_treatment_overview.tex <==
\begin{tikzpicture}[
  x=0.85cm,
  y=0.82cm,
  axis/.style={-{Stealth[length=2.2mm]}, line width=0.8pt},
  common/.style={black!75, line width=1.4pt},
  schedule/.style={line width=1.25pt},
  % 11 pt at native size becomes approximately 7.4 pt at one-column width.
  note/.style={font=\fontsize{11}{13}\selectfont, align=center, fill=white, inner sep=1pt},
  stage/.style={font=\fontsize{11}{13}\selectfont\bfseries, fill=white, inner sep=1.5pt}
]

% Fixed canvas shared with panel (b), ensuring aligned time axes.
\path[use as bounding box] (0.00,-0.35) rectangle (13.60,6.75);
\begin{pgfinterruptboundingbox}

% Qualitative axes.
\draw[line width=0.8pt] (0.55,0.15) -- (8.25,0.15);
\node[font=\large, fill=white, inner sep=1pt] at (8.70,0.15) {$\cdots$};
\draw[axis] (9.15,0.15) -- (12.35,0.15);
\draw[axis] (0.55,0.15) -- (0.55,6.25);
\node[note, anchor=north, inner sep=1pt, yshift=-2.5pt] at (6.45,0.15) {Time};
\node[note, rotate=90] at (0.20,3.20) {Temperature};

% Common part of every thermal cycle.
\draw[common]
  (0.85,0.78)
  -- (2.65,5.55)
  -- (4.05,5.55)
  -- (4.18,2.30)
  -- (8.25,2.30);
\draw[common] (9.15,2.30) -- (9.75,2.30);
\node[font=\large, fill=white, inner sep=1pt] at (8.70,2.30) {$\cdots$};

% Revised copy: allow a finite quenching interval so panel (b) can distinguish
% martensitic expansion during cooling from subsequent reheating for tempering.
% Interruption times and all stage durations are schematic.
\draw[schedule, blue!75!black]
  (4.18,2.30) -- (4.46,0.78)
  -- (4.66,1.55) -- (5.03,1.55) -- (5.18,0.95);

\draw[schedule, orange!85!black]
  (5.70,2.30) -- (5.98,0.78)
  -- (6.18,1.55) -- (6.55,1.55) -- (6.70,0.95);

\draw[schedule, green!60!black]
  (7.40,2.30) -- (7.68,0.78)
  -- (7.88,1.55) -- (8.25,1.55) -- (8.40,0.95);

\draw[schedule, teal!75!black]
  (9.75,2.30) -- (10.03,0.78)
  -- (10.23,1.55) -- (10.60,1.55) -- (10.75,0.95);

% Stage labels and schematic annotations.
\node[stage] at (3.35,5.88) {Austenitisation};
\node[stage] at (7.55,2.65) {Interrupted austempering};
\node[stage] (temperlabel) at (10.42,1.98) {Tempering};
\draw[-{Stealth[length=1.8mm]}, thin]
  (temperlabel.south) -- (10.42,1.58);

\draw[-{Stealth[length=2mm]}, thin]
  (4.70,3.25) -- (10.15,3.25)
  node[midway, above, note] {increasing interruption duration};

\node[stage, anchor=east] (quenchlabel) at (3.84,1.18) {Quenching};
\draw[-{Stealth[length=1.8mm]}, thin]
  (quenchlabel.east) -- (4.36,1.18);

\end{pgfinterruptboundingbox}
\end{tikzpicture}


==> Figures/Figure1_martensitic_expansion/label_generation_overview.tex <==
\begin{tikzpicture}[
  x=0.85cm,
  y=0.72cm,
  axis/.style={-{Stealth[length=2.2mm]}, line width=0.8pt},
  response/.style={black!80, line width=1.5pt},
  target/.style={densely dotted, line width=1.1pt},
  schedule/.style={line width=1.35pt},
  % 11 pt at native size becomes approximately 7.4 pt at one-column width.
  note/.style={font=\fontsize{11}{13}\selectfont, align=center, fill=white, inner sep=1pt},
  stage/.style={font=\fontsize{11}{13}\selectfont\bfseries, fill=white, inner sep=1.5pt}
]

\colorlet{levelzero}{blue!75!black}
\colorlet{levelthirty}{orange!85!black}
\colorlet{levelseventy}{green!60!black}
\colorlet{levelhundred}{teal!75!black}

% Fixed canvas shared with panel (a), ensuring aligned time axes.
\path[use as bounding box] (0.00,-0.35) rectangle (13.60,6.75);
\begin{pgfinterruptboundingbox}

% Qualitative axes.
\draw[line width=0.8pt] (0.55,0.35) -- (8.25,0.35);
\node[font=\large, fill=white, inner sep=1pt] at (8.70,0.35) {$\cdots$};
\draw[axis] (9.15,0.35) -- (12.35,0.35);
\draw[axis] (0.55,0.35) -- (0.55,6.25);
\node[note, anchor=north, inner sep=1pt, yshift=-2.5pt] at (6.45,0.35) {Time};
\node[note, rotate=90] at (0.20,3.20) {Relative length change};
\draw[axis] (12.10,2.00) -- (12.10,4.82);
\node[note, rotate=90] at (13.08,3.30) {Reference bainite fraction (\%)};

% Revised copy. Absolute heights, branch amplitudes and times are illustrative.
% The isothermal response is raised on the canvas to leave room for contraction
% followed by expansion accompanying martensitic transformation during quenching.
\draw[response]
  (0.85,1.05)
  -- (1.73,4.12)
  .. controls (1.78,4.43) and (1.83,4.60) .. (1.91,4.60)
  .. controls (2.01,4.60) and (2.07,4.36) .. (2.20,4.43)
  -- (2.65,5.82)
  -- (4.05,5.82)
  -- (4.18,2.00)
  .. controls (4.75,2.10) and (5.20,2.40) .. (5.70,2.74)
  .. controls (6.25,3.10) and (6.85,3.53) .. (7.40,3.74)
  .. controls (7.72,3.94) and (8.00,4.04) .. (8.25,4.10);
\draw[response]
  (9.15,4.43) .. controls (9.35,4.46) and (9.55,4.48) .. (9.75,4.48);
\node[font=\large, fill=white, inner sep=1pt] at (8.70,4.27) {$\cdots$};

% Representative normalised transformation levels used to select interruption points.
\draw[target, levelzero] (4.18,2.00) -- (12.10,2.00);
\fill[levelzero] (4.18,2.00) circle (1.7pt);
\draw[line width=0.7pt] (12.00,2.00) -- (12.20,2.00);
\node[note, text=levelzero, anchor=west] at (12.28,2.00) {5};

\draw[target, levelthirty] (5.70,2.74) -- (12.10,2.74);
\fill[levelthirty] (5.70,2.74) circle (1.7pt);
\draw[line width=0.7pt] (12.00,2.74) -- (12.20,2.74);
\node[note, text=levelthirty, anchor=west] at (12.28,2.74) {30};

\draw[target, levelseventy] (7.40,3.74) -- (12.10,3.74);
\fill[levelseventy] (7.40,3.74) circle (1.7pt);
\draw[line width=0.7pt] (12.00,3.74) -- (12.20,3.74);
\node[note, text=levelseventy, anchor=west] at (12.28,3.74) {70};

\draw[target, levelhundred] (9.75,4.48) -- (12.10,4.48);
\fill[levelhundred] (9.75,4.48) circle (1.7pt);
\draw[line width=0.7pt] (12.00,4.48) -- (12.20,4.48);
\node[note, text=levelhundred, anchor=west] at (12.28,4.48) {95};

% Coloured interrupted runs: thermal contraction, transformation expansion DURING
% quenching, further cooling, reheating/tempering, then the final cooling stage.
% The smaller expansion at higher bainite fractions is qualitative, not a fit.
% These times match the revised temperature panel.
\draw[schedule, levelzero]
  (4.18,2.00) -- (4.28,1.10)
  .. controls (4.30,1.10) and (4.33,1.95) .. (4.37,1.95)
  -- (4.46,1.75) -- (4.66,2.20)
  -- (5.03,2.20) -- (5.18,1.75);

\draw[schedule, levelthirty]
  (5.70,2.74) -- (5.80,1.84)
  .. controls (5.82,1.84) and (5.85,2.49) .. (5.89,2.49)
  -- (5.98,2.29) -- (6.18,2.74)
  -- (6.55,2.74) -- (6.70,2.29);

\draw[schedule, levelseventy]
  (7.40,3.74) -- (7.50,2.84)
  .. controls (7.52,2.84) and (7.55,3.14) .. (7.59,3.14)
  -- (7.68,2.94) -- (7.88,3.39)
  -- (8.25,3.39) -- (8.40,2.94);

\draw[schedule, levelhundred]
  (9.75,4.48) -- (9.85,3.58)
  .. controls (9.87,3.58) and (9.90,3.66) .. (9.94,3.66)
  -- (10.03,3.46) -- (10.23,3.91)
  -- (10.60,3.91) -- (10.75,3.46);

% Redraw the reference bainitic response above the coloured branches so that
% the monotonic transformation curve remains visually unambiguous.
\draw[white, line width=3.2pt]
  (4.18,2.00)
  .. controls (4.75,2.10) and (5.20,2.40) .. (5.70,2.74)
  .. controls (6.25,3.10) and (6.85,3.53) .. (7.40,3.74)
  .. controls (7.72,3.94) and (8.00,4.04) .. (8.25,4.10);
\draw[response]
  (4.18,2.00)
  .. controls (4.75,2.10) and (5.20,2.40) .. (5.70,2.74)
  .. controls (6.25,3.10) and (6.85,3.53) .. (7.40,3.74)
  .. controls (7.72,3.94) and (8.00,4.04) .. (8.25,4.10);

\draw[white, line width=3.2pt]
  (9.15,4.43) .. controls (9.35,4.46) and (9.55,4.48) .. (9.75,4.48);
\draw[response]
  (9.15,4.43) .. controls (9.35,4.46) and (9.55,4.48) .. (9.75,4.48);
\node[font=\large, fill=white, inner sep=1pt] at (8.70,4.27) {$\cdots$};

\fill[levelzero] (4.18,2.00) circle (1.7pt);
\fill[levelthirty] (5.70,2.74) circle (1.7pt);
\fill[levelseventy] (7.40,3.74) circle (1.7pt);
\fill[levelhundred] (9.75,4.48) circle (1.7pt);

\node[stage] (bainite) at (7.10,5.02) {Bainitic transformation};
\draw[-{Stealth[length=1.8mm]}, thin]
  (bainite.south) -- (6.62,3.35);

\node[stage] (martensite) at (7.25,1.04) {Martensitic transformation};
\draw[-{Stealth[length=1.8mm]}, thin]
  (martensite.north) -- (5.85,2.24);

\end{pgfinterruptboundingbox}
\end{tikzpicture}


==> Figures/histogram_patch_scale_bars.tex <==
% Vector overlays for the twelve 256 x 256-pixel patches in Figure 3.
% Shared calibration: 10 micrometres spans approximately 220 original pixels.
% Thus a 5-micrometre bar spans 110 original pixels, or 110/256 of a patch.
% The PGF renders each raster image at 1.05 inches wide before figure resizing:
% bar length = 1.05 * 110 / 256 = 0.451171875 inches.
% All coordinates use the original PGF canvas, so bars resize with the patches.
\newcommand{\histogrampatchscalebar}[2]{%
  \begin{pgfscope}%
    \pgftransformshift{\pgfqpoint{#1in}{#2in}}%
    \pgftransformshift{\pgfqpoint{0.555959in}{0.025in}}%
    \pgfsetfillcolor{white}%
    \pgfsetfillopacity{1}%
    \pgfpathrectangle{\pgfqpoint{-0.025in}{0in}}{\pgfqpoint{0.501171875in}{0.175in}}%
    \pgfusepath{fill}%
    \pgfsetstrokecolor{black}%
    \pgfsetstrokeopacity{1}%
    \pgfsetlinewidth{1pt}%
    \pgfsetdash{}{0pt}%
    \pgfpathmoveto{\pgfqpoint{0in}{0.05in}}%
    \pgfpathlineto{\pgfqpoint{0.451171875in}{0.05in}}%
    \pgfpathmoveto{\pgfqpoint{0in}{0.035in}}%
    \pgfpathlineto{\pgfqpoint{0in}{0.065in}}%
    \pgfpathmoveto{\pgfqpoint{0.451171875in}{0.035in}}%
    \pgfpathlineto{\pgfqpoint{0.451171875in}{0.065in}}%
    \pgfusepath{stroke}%
    \pgftext[x=0.225585938in,y=0.11in,base]{%
      \color{black}\normalfont\fontsize{7}{8.4}\selectfont\SI{5}{\micro\metre}}%
  \end{pgfscope}%
}
\histogrampatchscalebar{0.417216}{6.096394}%
\histogrampatchscalebar{1.494347}{6.096394}%
\histogrampatchscalebar{2.641477}{6.096394}%
\histogrampatchscalebar{3.718608}{6.096394}%
\histogrampatchscalebar{4.865739}{6.096394}%
\histogrampatchscalebar{5.942869}{6.096394}%
\histogrampatchscalebar{0.417216}{5.019263}%
\histogrampatchscalebar{1.494347}{5.019263}%
\histogrampatchscalebar{2.641477}{5.019263}%
\histogrampatchscalebar{3.718608}{5.019263}%
\histogrampatchscalebar{4.865739}{5.019263}%
\histogrampatchscalebar{5.942869}{5.019263}%

